Learning Parameterized Task Structure for Generalization to Unseen Entities

Real world tasks are hierarchical and compositional. Tasks can be composed of multiple subtasks (or sub-goals) that are dependent on each other. These subtasks are defined in terms of entities (e.g., "apple", "pear") that can be recombined to form new subtasks (e.g., "pickup apple", and "pickup pear"). To solve these tasks efficiently, an agent must infer subtask dependencies (e.g. an agent must execute "pickup apple" before "place apple in pot"), and generalize the inferred dependencies to new subtasks (e.g. "place apple in pot" is similar to "place apple in pan"). Moreover, an agent may also need to solve unseen tasks, which can involve unseen entities. To this end, we formulate parameterized subtask graph inference (PSGI), a method for modeling subtask dependencies using first-order logic with subtask entities. To facilitate this, we learn entity attributes in a zero-shot manner, which are used as quantifiers (e.g. "is_pickable(X)") for the parameterized subtask graph. We show this approach accurately learns the latent structure on hierarchical and compositional tasks more efficiently than prior work, and show PSGI can generalize by modelling structure on subtasks unseen during adaptation.

==> 05_experiments_new.tex <==
\cutsectionup
\section{Experiments}
\cutsectiondown

We aim to answer the following questions:
\begin{enumerate}
    \item Can PSGI \textit{generalize} to unseen evaluation tasks in zero-shot manner by transferring the inferred task structure?
    \item Does PSGI \textit{efficiently} infers the latent task structure compared to prior work (MSGI~\citep{sohn2020meta})?
    %\item Can PSGI \textit{generalize} to unseen subtasks with unseen entities using
%the inferred attributes?
\end{enumerate}

Additionally, we investigate the following questions in ablation experiments:
\begin{enumerate}
    \item Can PSGI \textit{generalize} to unseen subtasks with unseen entities using
the inferred attributes?
    \item How does the quality of the PSGI's prior affect transfer learning performance?
\end{enumerate}


\begin{figure*}[!h]
  \centering
  \includegraphics[trim=15 35 10 38,clip,width=1.0\textwidth]
  {figures/cooking_FSGI_inferred_graph.pdf}
  \caption{The inferred parameterized subtask graph by \fsgibf after 2000 timesteps in the \cook.
  Options are represented in rectangular nodes. Subtask completions and attributes are in oval nodes. A solid line represents a positive precondition / effect, dashed for negative.
  Ground truth attributes are included option/subtask parameters, however
  which attributes are used for which option preconditions is still hidden, which
  PSGI must infer.
  }
  \label{fig:cooking-pilp}
\end{figure*}
\begin{figure*}[!h]
  \centering
  \includegraphics[trim=15 10 10 50,clip,width=0.3\textwidth]
  {figures/transfer_performance_cooking_cumulative_reward_no_legend.pdf}
  \includegraphics[trim=15 10 10 50,clip,width=0.3\textwidth]
  {figures/transfer_performance_ai2thor_cumulative_reward_no_legend.pdf}
  \includegraphics[trim=15 10 10 50,clip,width=0.3\textwidth]
  {figures/transfer_performance_ETmining_cumulative_reward_no_legend.pdf}
  \\
  \includegraphics[trim=15 10 10 50,clip,width=0.3\textwidth]
  {figures/transfer_performance_cooking_success_no_legend.pdf}
  \includegraphics[trim=15 10 10 50,clip,width=0.3\textwidth]
  {figures/transfer_performance_ai2thor_success_no_legend.pdf}
  \includegraphics[trim=0 10 10 50,clip,width=0.3\textwidth]
  {figures/transfer_performance_ETmining_success.pdf}
  \vspace{-5pt}
  \caption{The adaptation curves in the \cook and \mine domains.
  \warning{PLACEHOLDER ai2thor result}
  }
  \label{fig:transfer_performance}
\end{figure*}

\cutsubsectionup
\subsection{Environments}
\cutsubsectiondown

We evaluate PSGI in the \thor environment \citep{ai2thor},
a simulated realistic indoor environment.
In our \thor environment, the agent is given a set of pre-trained
options and must cook various food objects in different kitchen layouts,
each containing possibly unseen objects.

We also evaluate PSGI in novel symbolic environments, \cook and \mine.
%
\cook is a simplified cooking environment with similar but simpler dynamics
to \thor. An example of the simplified \cook task is shown in Figure~\ref{fig:psgi-overview}.
The \mine domain is modelled after the open world video game Minecraft
and the domain introduced by~\citet{sohn2018hierarchical}.
Noteably, \mine is much more \textit{hierarchical} than \cook and \thor.
The agent must craft progressively newer equipment (\texttt{craft wood pickaxe},
\texttt{craft stone pickaxe}, etc.) in order to mine harder minerals, such
as diamond, like the video game. However, in \mine, the agent must also
generalize knowledge to different minerals (e.g. \texttt{silver} and \texttt{gold})
and craftables (e.g. \texttt{sword} and \texttt{pickaxe}).

\textbf{Tasks.}
\cook has a pool of 22 entities and 10 entities are chosen at random for each task.
Then, the subtasks and options are populated by replacing the parameters in parameterized subtasks and options by the sampled entities; \eg, we replace \texttt{X} and \texttt{Y} in the parameterized subtask \texttt{(pickup, X, Y)} by $\{\texttt{apple, cabbage, table}\}$ to populate nine subtasks. 
This results in around 320 options\todo{give exact number} and 100 subtasks\todo{give exact number}. The ground-truth attributes are also predefined in the templates, but is not available to the agent.
Similarly for \mine, we randomly sample 12 entities from a pool of 18 entities and populate around 180 subtasks\todo{give exact number} and 180 options\todo{give exact number} for each task.
The reward is assigned at random to one of the subtasks that have the largest critical path length, where the critical path length is the minimum number of options to be executed to complete each subtask. See the appendix for more details on the tasks.

\textbf{Observations.}
At each time step, the agent observes the completion and eligibility vectors (see \textit{Parameterized Subtask Graph Problem} section for definitions) and the corresponding embeddings. The subtask and option embeddings are the concatenated vector of the embeddings of its entities; \eg, for \texttt{pickup, apple, table} the embedding is $[f(\texttt{pickup}), f(\texttt{apple}), f(\texttt{table})]$ where $f(\cdot)$ can be an image or language embeddings. In experiment, we used 50 dimensional GloVE word embeddings~\citep{pennington2014glove} as the embedding function $f(\cdot)$.

\cutsubsectionup
\subsection{Baselines}
\cutsubsectiondown

\begin{itemize}
   \setlength{\itemsep}{0pt}
    \item \msgi is the \msgiorg~\citep{sohn2020meta} agent modified to be capable of solving our \cook and \mine tasks. We augmented \msgiorg with an effect model, separate subtasks and options in the ILP algorithm, and replace the GRProp with cyclic GRProp, a modified version of GRProp that can run with cycles in the subtask graph.
    %\item \rlrl~\cite{duan2016rl} trains a recurrent model over the training tasks to quickly adapt to given task as it is rolled out.
    \item \hrl~\citep{andreas2017modular}\footnote{In~\citet{andreas2017modular} this agent was referred as Independent model.} is the option-based hierarchical reinforcement learning agent. It is an actor-critic model over the pre-learned options.
    \item \random agent randomly executes any eligible option.
\end{itemize}
%
We meta-train \fsgibf on training tasks and meta-eval on evaluation tasks to test its adaptation efficiency and generalization ability.
We train \hrl on evaluation tasks to test its adaptation (\ie, learning) efficiency.
We evaluate \random baseline on evaluation tasks to get a reference performance.
We use the same recurrent neural network with self-attention-mechanism so that the agent can handle varying number of (unseen) parameterized subtasks and options depending on the tasks. See the appendix for more details on the baselines.

\cutsubsectionup
\subsection{Zero-/Few-shot Transfer Learning Performance}
\cutsubsectiondown

\textbf{Zero-shot learning performance.} \Cref{fig:transfer_performance} compares the zero-shot and few-shot transfer learning performance on \mine and \cook domains.
% fsgi vs msgi+
First, \fsgibf achieves over 50 and 30\% success rate on \cook and \mine domain without observing any samples (\ie, x-axis value = 0) in unseen evaluation tasks. This indicates that the parameterized subtask graph effectively captures the shared task structure, and the inferred attributes generalizes well to unseen entities in zero-shot manner. Note that \msgi, \hrl, and \random baselines have no ability to transfer its policy from training tasks to unseen evaluation tasks.
We note that \msgi has no mechanism for generalizing to the tasks with unseen entities.

\textbf{Few-shot learning performance.} In~\Cref{fig:transfer_performance}, \fsgibf achieves over 90 and 80\% success rate on \cook and \mine domains respectively after only 1000 steps of adaptation, while other baselines do not learn any meaningful policy except \msgi in \cook. This demonstrates that the parameterized subtask graph enables \fsgibf to share the experience of similar subtasks and options (\eg, \texttt{pickup X on Y} for all possible pairs of \texttt{X} and \texttt{Y}) such that the sample efficiency is increased by roughly the factor of number of entities compared to using subtask graph in \msgi.

\cutsubsectionup
\subsection{Comparison on Task Structure Inference}
\cutsubsectiondown

We ran \fsgibf and \msgi in the \cook and \mine, inferring the latent
subtask graphs %every 50 timesteps, 
for 2000 timesteps. The inferred graphs at 2000 timesteps are shown in~\Cref{fig:cooking-pilp}.
In the interest of space, we have shown the inferred graph by \msgi in the appendix in~\Cref{fig:cooking-pilp-msgi}.
\fsgibf infers the parameterized graph using first-order logic, and thus it is more compact. On the other hand, \msgi infers the subtask graph without parameterizing out the shared structure, resulting in non-compact graph with hundreds of subtasks and options. Moreover, graph inferred by \fsgibf has 0\% error in precondition and effect model inference. The graph inferred by \msgi has 38\% error in the preconditions (the six options that \msgi completely failed to infer any precondition are not shown in the figure for readability).
The result shows that the parameterized graph can infer the task structure much more efficiently than the subtask graph by sharing the experiences of different options using the parameterized options and subtasks.


\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.30\textwidth]{figures/ablation_prior_cooking_cumulative_reward_no_legend.pdf}
  \includegraphics[width=0.30\textwidth]{figures/ablation_prior_ai2thor_cumulative_reward_no_legend.pdf}
  \includegraphics[width=0.30\textwidth]{figures/ablation_prior_ETmining_cumulative_reward_no_legend.pdf}
  \\
  \includegraphics[width=0.30\textwidth]{figures/ablation_prior_cooking_success_no_legend.pdf}
  \includegraphics[width=0.30\textwidth]{figures/ablation_prior_ai2thor_success_no_legend.pdf}
  \includegraphics[width=0.30\textwidth]{figures/ablation_prior_ETmining_success.pdf}
  \caption{The adaptation curve of \fsgibf trained with different priors. Priors were
  trained in the training tasks of \cook and \mine domains respectively
  for $T_\text{prior}= 100, 500,$ and $2000$ timesteps.
  }
  \label{fig:ablation_prior}
\end{figure*}

\subsection{Ablation: Zero Shot Learning Attributes}
In our experiments, we assume the first entity of every subtask and option
serves as a ``verb'' entity (e.g. \texttt{pickup}, \texttt{cook}, etc.).
We assume there is there is no shared structure across subtasks and options with
different verbs.

As described in section~\ref{sec:zero-shot-learning-attributes},
(when attributes are not provided), we infer attributes from an exhaustive
powerset of all possible features on seen parameters.
The attributes that are used for the graph are then likely to be semantically
meaningful, as the decision tree selects the most efficient features.
Hence, to test whether PSGI is generalizable, we can evaluate \textit{whether
attributes are accurately inferred} for unseen parameters when only given the ground truth attributes
on seen parameters (given that PSGI will infer the ground truth for the seen parameters).

We measure the generalization error of PSGI if some ``weak" signal is provided
through parameters. We suppose the word labels for options and subtasks are provided in \cook.
I.e.\ the words for parameters ``pickup", ``apple", etc. are known.
Then, we can infer low level (but semantically meaningful) features from these words
by using \textit{word embeddings} to encode the parameters~\citep{pennington2014glove}.
We choose to use 50 dimensional GloVE word embeddings from~\citet{pennington2014glove}.
We then evaluate by measuring the accuracy of attributes for \textbf{20} additional
unseen test parameters, all words related to kitchens and cooking. We show the
results in Table~\ref{tab:attribute-inf-accuracy}.

%mining 0.8792857143	0.01518030264
%cooking 0.9486111111	0.01041455334
%ai2thor 0.8226535627	0.03948472028

\begin{table}[]
    \centering
    \begin{tabular}{l|r}
        Environment &
        \begin{tabular}{@{}c@{}}Attribute Generalization \\ Accuracy\end{tabular}\\
        \hline
        \cook & $94.9 \pm 1.0$\%\\
        \mine & $87.9 \pm 1.5$\% \\
        \thor & $82.3 \pm 3.9$\%
    \end{tabular}
    \caption{We evaluate the generalization accuracy of PSGI on unseen test entities
    in each environment. For each ground truth attribute, we evaluate
    whether PSGI accurately labels the unseen test entity correctly.
    We show the average accuracy over each ground truth attribute in environments.
    }
    \label{tab:attribute-inf-accuracy}
\end{table}
From these results, we can extrapolate that at least \textbf{70\%} of edges
(on unseen entities) in the predicate subtask graph using these attributes are accurate.

\subsection{Ablation: Effect of the Prior}
As described in the Task Transfer and Adaptation section,
in PSGI, the training phase is used to learn a prior parameterized subtask
graph, $\widehat{\FG}_\text{prior}$.
$\widehat{\FG}_\text{prior}$ is then used in an ensemble with the the test policy's
learned graph $\widehat{\FG}_\text{test}$.
Then, we can infer that the more accurate $\widehat{\FG}_\text{prior}$ is, the better
the transfer policy will perform.
To study this, we varied the number of timesteps used to learn the priors
in the \cook and \mine domains. We trained priors $T_\text{prior}= 100, 500,$ and $2000$ timesteps
respectively, shown in ~\Cref{fig:ablation_prior}.

In the \cook domain, we can see that when $T_\text{prior}$ is higher,
the average return and success rate increases.
However, in the \mine domain, we see no obvious correlation between $T_\text{prior}$ and performance.
We reason that this may be from a number of factors --- the prior graphs may not have
significant difference between $T_\text{prior} = 100, 500,$ and $2000$ timesteps,
or that $\widehat{\FG}_\text{prior}$ is significantly different from the latent
parameterized subtask graph during testing, rendering the prior less useful.

==> math_commands.tex <==
\usepackage{xspace}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}

\DeclareMathOperator*{\argmax}{argmax} % thin space, limits underneath in displays
\DeclareMathOperator*{\argmin}{argmin} % thin space, limits underneath in displays


==> old/04_related_work.tex <==
\section{Related Work}

\paragraph{Subtask Graph Inference.} The subtask graph inference (SGI) framework~\cite{sohn2018hierarchical,sohn2020meta} assumes that a task consists of multiple base subtasks, such that the entire task can be solved by completing a set of subtasks in the right order. Then, it has been shown that SGI can efficiently solve the complex task by explicitly inferring the precondition relationship between subtasks in the form of a graph using an inductive logic programming (ILP) method. The inferred subtask graph is in turn fed to an execution policy that can predict the optimal sequence of subtasks to be completed to solve the given task.

However, the proposed SGI framework is limited to a single task; the knowledge learned in one task cannot be transferred to another. This limits the SGI framework such that
does not scale well to compositional tasks, and cannot generalize to unseen tasks.
We extend the SGI framework by modeling \textit{parameterized} subtasks and options,
which encode relations between tasks to allow efficient and general learning.
In addition, we generalize the SGI framework by learning an effect model --
In the SGI framework it was assumed that for each subtask there is a corresponding option, that
completes that subtask (and does not effect any other subtask).
%This assumption
%is unrealistic when there options must also be parameterized in the combinatorial task
%structure, and there exist subtasks that cannot be completed \textit{without un-completing another} (e.g. \texttt{Pickup} and \texttt{Place} in Figure~\ref{fig:psgi-overview}).
%
\paragraph{Compositional Task Generalization.}
Prior work has also tackled compositional generalization in a symbolic manner~\cite{loula2018rearranging,andreas2017modular,oh2017zero}.
\cite{loula2018rearranging} test compositional generalization of
natural language sentences in recurrent neural networks.
\cite{andreas2017modular,oh2017zero} tackle compositional task generalization
in an \textit{instruction following} context, where an agent
is given a natural language instruction describing the task the agent must complete
(e.g.\ ``pickup apple").
These works use \textit{analogy making} to learn policies that can execute
instructions by analogy (e.g.\ ``pickup $X$").
However, these works construct policies on the \textit{option level} --
they construct policies that can execute ``pickup $X$" on different $X$ values.
They also do not consider hierarchical structure for the order which options should
be executed (as the option order is given in instruction).
Our work aims to learn these analogy-like relations at a between-options level,
where certain subtasks must be completed before another option can be executed.

\paragraph{Classical Planning.}
At a high level, a parameterized subtask graph $\FG$ is equivalent to a STRIPS planning domain~\cite{fikes1971strips} with an attribute model add-on~\cite{frank2003constraint}.
\iffalse
\textit{Operators} in STRIPS correspond to options in $\FG$. The symbolic state space
in STRIPS corresponds to subtask completion in $\FG$. Arguments to operators and states
are similar to parameters in $\FG$.
Most work in classical planning focuses on how to use a domain specification to instantiate
a solution plan, equivalent to our reward maximization phase.
A viable option \psgi{} is to replace our test policy with a classical planner using our inferred
parameterized subtask graph.
\fi
Prior work in classical planning has proposed to learn STRIPS domain specifications (action schemas) through given trajectories (action traces)~\cite{suarez2020strips,mehta2011autonomous,walsh2008efficient,zhuo2010learning}.
Our work differs from these in 3 major ways:
1. \psgi{} learns an \textit{attribute} model, which is crucial to generalizing
compositional tasks with components of different behaviors.
2. We evaluate \psgi{} on more hierarchical domains, where prior work
has evaluated on pickup-place/travelling classical planning problems, which admit
flat structure.
3. We evaluate \psgi{} on generalization, where there may exist subtasks and options
that are not seen during adaptation.
%3. PSGI takes an \textit{active} approach to learning the latent graph stucture.
%PSGI updates the adaptation policy to explore the environment more efficiently.
%Prior work assumes that the trajectories are given.\todo{double check this (probably can't make this claim}

==> old/05_experiments.tex <==
\section{Experiments}

We aim to answer the following questions:
\begin{enumerate}
    \item Can PSGI \textit{generalize} to unseen evaluation tasks in zero-shot manner by transferring the inferred task structure?
    \item Does PSGI \textit{efficiently} infers the latent task structure compared to prior work (MSGI~\cite{sohn2020meta})?
    %\item Can PSGI \textit{generalize} to unseen subtasks with unseen entities using
%the inferred attributes?
\end{enumerate}

\begin{figure*}[!h]
  \centering
  \includegraphics[trim=15 35 10 38,clip,width=1.0\textwidth]
  {figures/cooking_FSGI_inferred_graph.pdf}
  \caption{The inferred parameterized subtask graph by \fsgibf after 2000 timesteps in the \cook.
  Options are represented in rectangular nodes. Subtask completions and attributes
  are are in oval nodes. A solid line represents a positive precondition / effect, dashed for negative.
  Ground truth attributes are included option/subtask parameters, however
  which attributes are used for which option preconditions is still hidden, which
  PSGI must infer.
  }
  \label{fig:cooking-pilp}
\end{figure*}
\begin{figure*}[!h]
  \centering
  \includegraphics[trim=15 10 10 50,clip,width=0.245\textwidth]
  {figures/transfer_performance_cooking_cumulative_reward_no_legend.pdf}
  \includegraphics[trim=15 10 10 50,clip,width=0.245\textwidth]
  {figures/transfer_performance_cooking_success_no_legend.pdf}
  \includegraphics[trim=15 10 10 50,clip,width=0.245\textwidth]
  {figures/transfer_performance_ETmining_cumulative_reward_no_legend.pdf}
  \includegraphics[trim=0 10 10 50,clip,width=0.245\textwidth]
  {figures/transfer_performance_ETmining_success.pdf}
  \vspace{-5pt}
  \caption{The adaptation curves in the \cook and \mine domains.
  }
  \label{fig:transfer_performance}
\end{figure*}

\subsection{Environments}
We evaluate PSGI in a novel symbolic environment, \cook and \mine.
%
An example of the simplified \cook task is shown in Figure~\ref{fig:psgi-overview}.
For each task, we manually define the parameterized subtask graph in terms parameterized subtasks, options, and attributes in first-order logic form. Then, the subtask graph can be built by replacing each predicate with a set of task-specific entities.
Each task is randomized by randomly sampling the entities from the entity pool.
The entity pool for training and evaluation tasks are different such that the agent should be able to generalize to unseen entities to solve the evaluation tasks in zero-shot setting.
% size of the task

\textbf{Tasks.}
\cook has a pool of 22 entities and 10 entities are chosen at random for each task.
Then, the subtasks and options are populated by replacing the parameters in parameterized subtasks and options by the sampled entities; \eg, we replace \texttt{X} and \texttt{Y} in the parameterized subtask \texttt{(pickup, X, Y)} by $\{\texttt{apple, cabbage, table}\}$ to populate nine subtasks. 
This results in around 320 options and 100 subtasks. The ground-truth attributes are also predefined in the templates, but is not available to the agent.
Similarly for \mine, we randomly sample 12 entities from a pool of 18 entities and populate around 180 subtasks and 180 options for each task.
The reward is assigned at random to one of the subtasks that have the largest critical path length, where the critical path length is the minimum number of options to be executed to complete each subtask. See the appendix for more details on the tasks.

\textbf{Observations.}
At each time step, the agent observes the completion and eligibility vectors (see \textit{Parameterized Subtask Graph Problem} section for definitions) and the corresponding embeddings. The subtask and option embeddings are the concatenated vector of the embeddings of its entities; \eg, for \texttt{pickup, apple, table} the embedding is $[f(\texttt{pickup}), f(\texttt{apple}), f(\texttt{table})]$ where $f(\cdot)$ can be an image or language embeddings. In experiment, we used 50 dimensional GloVE word embeddings~\citep{pennington2014glove} as the embedding function $f(\cdot)$.

\subsection{Baselines}
\begin{itemize}
   \setlength{\itemsep}{0pt}
    \item \msgi is the \msgiorg~\cite{sohn2020meta} agent modified to be capable of solving our \cook and \mine tasks. We augmented \msgiorg with an effect model, separate subtasks and options in the ILP algorithm, and replace the GRProp with cyclic GRProp, a modified version of GRProp that can run with cycles in the subtask graph.
    %\item \rlrl~\cite{duan2016rl} trains a recurrent model over the training tasks to quickly adapt to given task as it is rolled out.
    \item \hrl~\cite{andreas2017modular}\footnote{In~\cite{andreas2017modular} this agent was referred as Independent model.} is the option-based hierarchical reinforcement learning agent. It is an actor-critic model over the pre-learned options.
    \item \random agent randomly executes any eligible option.
\end{itemize}
%
We meta-train \fsgibf on training tasks and meta-eval on evaluation tasks to test its adaptation efficiency and generalization ability.
We train \hrl on evaluation tasks to test its adaptation (\ie, learning) efficiency.
We evaluate \random baseline on evaluation tasks to get a reference performance.
We use the same recurrent neural network with self-attention-mechanism so that the agent can handle varying number of (unseen) parameterized subtasks and options depending on the tasks. See the appendix for more details on the baselines.

\subsection{Zero-/Few-shot Transfer Learning Performance}

\textbf{Zero-shot learning performance.} \Cref{fig:transfer_performance} compares the zero-shot and few-shot transfer learning performance on \mine and \cook domains.
% fsgi vs msgi+
First, \fsgibf achieves over 50 and 30\% success rate on \cook and \mine domain without observing any samples (\ie, x-axis value = 0) in unseen evaluation tasks. This indicates that the parameterized subtask graph effectively captures the shared task structure, and the inferred attributes generalizes well to unseen entities in zero-shot manner. Note that \msgi, \hrl, and \random baselines have no ability to transfer its policy from training tasks to unseen evaluation tasks.
We note that \msgi has no mechanism for generalizing to the tasks with unseen entities.

\textbf{Few-shot learning performance.} In~\Cref{fig:transfer_performance}, \fsgibf achieves over 90 and 80\% success rate on \cook and \mine domains respectively after only 1000 steps of adaptation, while other baselines do not learn any meaningful policy except \msgi in \cook. This demonstrates that the parameterized subtask graph enables \fsgibf to share the experience of similar subtasks and options (\eg, \texttt{pickup X on Y} for all possible pairs of \texttt{X} and \texttt{Y}) such that the sample efficiency is increased by roughly the factor of number of entities compared to using subtask graph in \msgi.

\subsection{Comparison on Task Structure Inference}
We ran \fsgibf and \msgi in the \cook and \mine, inferring the latent
subtask graphs %every 50 timesteps, 
for 2000 timesteps. The inferred graphs at 2000 timesteps are shown in~\Cref{fig:cooking-pilp}.
In the interest of space, we have shown the inferred graph by \msgi in the appendix in~\Cref{fig:cooking-pilp-msgi}.
\fsgibf infers the parameterized graph using first-order logic, and thus it is more compact. On the other hand, \msgi infers the subtask graph without parameterizing out the shared structure, resulting in non-compact graph with hundreds of subtasks and options. Moreover, graph inferred by \fsgibf has 0\% error in precondition and effect model inference. The graph inferred by \msgi has 38\% error in the preconditions (the six options that \msgi completely failed to infer any precondition are not shown in the figure for readability).
The result shows that the parameterized graph can infer the task structure much more efficiently than the subtask graph by sharing the experiences of different options using the parameterized options and subtasks.


==> old/figure2_captions_old.tex <==
\begin{figure*}[h!]
\begin{subfigure}[b]{\textwidth}
  \centering
  \includegraphics[trim=10 30 10 30,clip,width=0.8\textwidth]{figures/PSGI-PILP-precond-v1.1.pdf}
  \caption{Parameterized Precondition Inference via inductive logic programming.
  We run precondition inference for every option and show $D_X$ as an example.
  \textbf{1.} The first table is built from the agent's trajectory ($x$ is the subtask completion, $e$ the option eligibility).
  \textbf{2.} We build the second table, the ``augmented'' trajectory by substituting
  $X$ into all possible subtask completions, $A_X, B_X$, and inferred attributes $f, g$.
  \textbf{3.} We train a decision tree over the table, to infer the relation $x_\text{aug} \to D_x$.
  \textbf{4.} We translate the decision tree into an equivalent predicate boolean expression,
  which is one part of the inferred parameratized subtask graph $\widehat{\FG}$.
  }
  \label{fig:pilp-precond-overview}
\end{subfigure}
\iffalse
\begin{subfigure}[b]{\textwidth}
  \centering
  \includegraphics[trim=10 50 10 30,clip,width=\textwidth]{figures/PSGI-PILP-effect-v1.1.pdf}
  \caption{Parameterized Effect Inference.
  We run effect inference for every option and $D_X$ as an example.
  \textbf{1.} The first table is built from the agent's trajectory ($x_t, o_t$ is the subtask
  completion and option executed at time $t$).
  \textbf{2.} We build the second table, the ``augmented'' trajectory by substituting
  $X$ into all possible subtask completions, $A_X, B_X$, and restricting the table to
  only row where $o_t = D_X$.
  \textbf{3.} We infer option dynamics, $(x_t, o_t) \mapsto x_{t+1}$, by calculating the simple aggregated difference between subtask completion
  before and after $D_X$, $\Delta(x_{t,\text{aug}}, x_{t+1,\text{aug}})$.
  }
  \label{fig:pilp-effect-overview}
\end{subfigure}
\fi
  \caption{An overview of our approach for estimating the parameterized subtask graph $\widehat{\FG}$ in a simple environment with subtasks $A, B$ and options $C, D, E$.
  Each subtask and option has a parameter 0 or 1. Note by inferring the parameterized
  precondition and effects, we can infer the behavior unseen subtasks and options such as $D_2$.\todo{too big? Think about shrinking it}}
  \label{fig:pilp-overview}
\end{figure*}
